Continuous Cost Aggregation for Dual-Pixel Disparity Extraction

Recent works have shown that depth information can be obtained from Dual-Pixel (DP) sensors. A DP arrangement provides two views in a single shot, thus resembling a stereo image pair with a tiny baseline. However, the different point spread function (PSF) per view, as well as the small disparity range, makes the use of typical stereo matching algorithms problematic. To address the above shortcomings, we propose a Continuous Cost Aggregation (CCA) scheme within a semi-global matching framework that is able to provide accurate continuous disparities from DP images. The proposed algorithm fits parabolas to matching costs and aggregates parabola coefficients along image paths. The aggregation step is performed subject to a quadratic constraint that not only enforces the disparity smoothness but also maintains the quadratic form of the total costs. This gives rise to an inherently efficient disparity propagation scheme with a pixel-wise minimization in closed-form. Furthermore, the continuous form allows for a robust multi-scale aggregation that better compensates for the varying PSF. Experiments on DP data from both DSLR and phone cameras show that the proposed scheme attains state-of-the-art performance in DP disparity estimation.

==> Figs/CMP_SGM_CSGM.tex <==
\begin{figure}[t]
  \begin{center}
   \begin{tabular}{c@{~~}c@{}c@{}c@{}}
      
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/005_B.jpg} &
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/035_B.jpg} &
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/075_B.jpg} \\
      \small{(a) Left image} & \small{(b) SGM} &  \small{(c) CSGM} \\

      
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/005_B.jpg} &
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/035_B.jpg} &
      \includegraphics[width=0.33\linewidth]{\Figs/DSLR_Quantitive/Images/075_B.jpg} \\
      \small{(d) Cross-section} & \small{(e) SGM - error} &  \small{(f) CSGM - error}

    \end{tabular}
    \end{center}
 \caption{Comparison between SGM and CSGM: We compare between SGM and CSGM without any post-processing and the same cost function. (a) Input image. (b) SGM result. (c) CSGM result. (d) Cross section of disparity. (e) 0.5 pixel error map - SGM, white is correct classifed pixels. (e) 0.5 pixel error - CSGM. }
 \label{fig:sgm_vs_csgm}
\end{figure}


==> Figs/PIXEL_result_main2.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c}

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im14.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT14.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST14.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN14.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/14.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/14.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/11.png} \\

      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/12.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/7.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im23.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT23.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST23.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN23.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/23.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/23.png} \\

      Image & GT & SDoF~\cite{Wadhwa_SIGGRAPH2018_syntheticDoF} & LDP~\cite{Garg-ICCV2019-learningDual} & CCA & CCA + filter
    \end{tabular}
    \end{center}
 \caption{Additional results on Google Pixel phone. Including results from the DNN used in~\cite{Garg-ICCV2019-learningDual}, where the network outputs depth instead of disparity like CCA and SDoF\cite{Wadhwa_SIGGRAPH2018_syntheticDoF}. Both SDoF and LDP were taken from~\cite{Garg-ICCV2019-learningDual}.}%\sagi{add that the DNN results are depth and not disparity. Also, maybe we should refer the reader to the radial artifacts that are due to being uncalibrated disparity} \Monin{Radial artifacts are in Fig 1, commented on depth (also appears in text)}}
 \label{fig:PIXEL_result_main2}
\end{figure*}


==> Figs/PIXEL_result_main3.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c}

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im16.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT16.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST16.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN16.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/16.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/16.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im18.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT18.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST18.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN18.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/18.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/18.png} \\

      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im21.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT21.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST21.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN21.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/21.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/21.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im20.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT20.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST20.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN20.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/20.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/20.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/Images/Im22.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/GT/GT22.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/SDOF/ST22.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/LDP/NN22.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM/22.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Pixel_result/CSGM_filter/22.png} \\

      Image & GT  & SDoF~\cite{Wadhwa_SIGGRAPH2018_syntheticDoF} & LDP~\cite{Garg-ICCV2019-learningDual} & CCA & CCA + filter
    \end{tabular}
    \end{center}
\caption{Additional results on Google Pixel phone. Including results from the DNN used in~\cite{Garg-ICCV2019-learningDual}, where the network outputs depth instead of disparity like CCA and SDoF\cite{Wadhwa_SIGGRAPH2018_syntheticDoF}. Both SDoF and LDP were taken from~\cite{Garg-ICCV2019-learningDual}.} \label{fig:PIXEL_result_main3}
\end{figure*}


==> Figs/STEREO_failure.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c}

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM7.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM11.png} \\

      (a) Image & (b) GT & (c) CSGM & (d) SGM  & (e) CSGM \textbackslash w filter & (f) SGM \textbackslash w filter
    \end{tabular}
    \end{center}
 \caption{Results on middlebury training dataset at quarter resolution - SGM outperforms C-SGM: In both scenarios SGM outperforms C-SGM by approx. 5\% for metrics of number of bad pixels, where SGM more accurately detects smooth regions texture less regions such as the wall in both images and the chair seat in the second row. (a) Left input image. (b) Ground truth disparity images. (c) Results of CSGM without post-processing filter. (d) Results of SGM without post-processing filter. (e) Results of CSGM with post-processing filter (f) Results of SGM with post-processing filter. For both algorithms the same post-processing filter was applied.}
 \label{fig:Stereo_failure}
\end{figure*}


==> Figs/STEREO_failure2.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c}

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT7.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter7.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM7.png} & 
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_CSGM/CSGM_mask_1pix7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_SGM/SGM_mask_1pix7.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT11.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter11.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_CSGM/CSGM_mask_1pix11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_SGM/SGM_mask_1pix11.png} \\

      (a) Image & (b) GT & (c) CSGM \textbackslash w filter & (d) SGM \textbackslash w filter & (e) CSGM-bad px.1 & (f) SGM-bad px.1
    \end{tabular}
    \end{center}
 \caption{Results on middlebury training dataset at quarter resolution - SGM outperforms C-SGM: In both scenarios SGM outperforms C-SGM by approx. 5\% for metrics of number of bad pixels, where SGM more accurately detects smooth regions texture less regions such as the wall in both images and the chair seat in the second row. (a) Left input image. (b) Ground truth disparity images. (c) Results of CSGM with post-processing filter (d) Results of SGM with post-processing filter. For both algorithms the same post-processing filter was applied. (e) CSGM result: Image of pixels within distance of 1 disparity pixel from GT. Yellow pixels are correct classified pixels. (f) SGM result: Image of pixels within distance of 1 disparity pixel from GT. }
 \label{fig:Stereo_failure_detail}
\end{figure*}


==> Figs/STEREO_supp_res.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c}

      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_2.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT2.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter2.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter2.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM2.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM2.png} \\

      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_4.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT4.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter4.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter4.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM4.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM4.png} \\

      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM12.png} &
      \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM12.png} \\
      
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM11.png} \\ 
      
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT11.png} &
    %   % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter11.png} &
    %   % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_CSGM/CSGM_mask_1pix11.png} &
    %   \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_SGM/SGM_mask_1pix11.png} \\

      (a) Image & (b) GT & (c) CCA  & (d) SGM  & (e) CCA + filter & (f) SGM + filter
    \end{tabular}
    \end{center}
 \caption{Additional results on middlebury training dataset at quarter resolution, showing our algorithm performs similar to SGM.} %\Monin{I removed the image} \sagi{In the last row, the floor results for the CSGM is very noisy. It shouldn't be like that and indicates an issue. Our main point was that we produce smooth sub-pixel results, but it looks noisier compared to SGM} \Monin{This is an area with a lot of repeated texture - so the algorithm doesn't do as good as SGM (the entire floor is just repeated texture). Also the range of disparity is about 80 pixels, so noise is not sub-pixel smooth but points with high confidence and wrong integer disparity}}
 \label{fig:Stereo_result_supp}
\end{figure*}


==> Figs/STEREO_table_occ_res.tex <==
\begin{table}[b!]   
\begin{tabular}{|c|c|c|c|c|}
    \hline
	Method & Bad px & Bad px &  Bad px  & RMSE \\ 
 	 & 0.5 $[\%]$ &  1 $[\%]$ &   2 $[\%]$ &  \\ 

    \hline
    SGM & 36.2 & 27.5 & 21.6 & 8.8  \\
    \hline 
    CCA & 37.3 & 27.9 & 22 & 14 \\ 
    \hline
    SGM $+$ filter& 33.8 & 24.4 & 18.3 & 5.9  \\
    \hline 
    CCA $+$ filter& 34.3 & 25.2 & 18.6 & 5.6  \\ 
    \hline
\end{tabular}
\caption{Comparison of SGM and CCA performance on all pixels of middle-bury training dataset. } 
\label{tab:Stereo_res_occ}
\end{table}
%\end{figure}

==> sections/STEREO_failure2.tex <==
\begin{figure*}[t]
  \begin{center}
   \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c}

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT7.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter7.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM7.png} & 
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_CSGM/CSGM_mask_1pix7.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_SGM/SGM_mask_1pix7.png} \\

       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/images/im_11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/GT/GT11.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_no_filter_no_mask/CSGM_no_filter11.png} &
       % \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_no_filter_no_mask/SGM_no_filter11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/csgm_filter_no_mask/CSGM11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/sgm_filter_no_mask/SGM11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_CSGM/CSGM_mask_1pix11.png} &
       \includegraphics[width=0.15\linewidth]{\Figs/Stereo_CSGM_vs_SGM/mask_SGM/SGM_mask_1pix11.png} \\

      (a) Image & (b) GT & (c) CSGM \textbackslash w filter & (d) SGM \textbackslash w filter & (e) CSGM-bad px.1 & (f) SGM-bad px.1
    \end{tabular}
    \end{center}
 \caption{Results on middlebury training dataset at quarter resolution - SGM outperforms C-SGM: In both scenarios SGM outperforms C-SGM by approx. 5\% for metrics of number of bad pixels, where SGM more accurately detects smooth regions texture less regions such as the wall in both images and the chair seat in the second row. (a) Left input image. (b) Ground truth disparity images. (c) Results of CSGM with post-processing filter (d) Results of SGM with post-processing filter. For both algorithms the same post-processing filter was applied. (e) CSGM result: Image of pixels within distance of 1 disparity pixel from GT. Yellow pixels are correct classified pixels. (f) SGM result: Image of pixels within distance of 1 disparity pixel from GT. }
 \label{fig:Stereo_failure_detail}
\end{figure*}

